Scalable Routing in a City-Scale Wi-Fi Network for Disaster Recovery

In this paper, we present a new city-scale decentralized mesh network system suited for disaster recovery and emergencies. When wide-area connectivity is unavailable or significantly degraded, our system, MapMesh, enables static access points and mobile devices equipped with Wi-Fi in a city to route packets via each other for intra-city connectivity and to/from any nodes that might have Internet access, e.g., via satellite. The chief contribution of our work is a new routing protocol that scales to millions of nodes, a significant improvement over prior work on wireless mesh and mobile ad hoc networks. Our approach uses detailed information about buildings from widely available maps--data that was unavailable at scale over a decade ago, but is widely available now--to compute paths in a scalable way.

==> sections/evaluation.tex <==
\section{Evaluation}\label{sec-evaluation}


We evaluate \name using city-scale simulations and hardware testbed.
For simulations, we answer the questions below:
\begin{itemize}[leftmargin=*]
\item Scalability for large-scale city topologies (\S\ref{subsec-evaluation-2}) 
\item Sensitivity of parameters (\S\ref{subsec-evaluation-3})
\item Component-wise study (\S\ref{subsec-evaluation-4})
\end{itemize}
% For the hardware testbed, we focus on:
% \begin{itemize}[leftmargin=*]
%     \item \textbf{Large scale emulation}: How does the simulated performance of our algorithm change when using real packet transmissions and receptions, versus using an RF model?
%     \item \jl{Should we report packet loss rates measured by the testbed?}
%     %\item \textbf{Packet loss rate}: What is the approximate packet loss rate that occurs between access points in the same building and access points in different buildings?
%     \item \textbf{Performance}: What are the performance demands of our algorithm? Will our algorithm perform well on commodity hardware?
%     \item \textbf{Large scale emulation}: How does the simulated performance of our algorithm change when using real packet transmissions and receptions, versus using an RF model?
% \end{itemize}



\begin{figure*}[t]
    \centering
    \begin{subfigure}[h]{0.3\linewidth}
        \includegraphics[width=\linewidth]{figs/loss-rates/network-graph.png}
        \caption{Effective adjacency graph of nodes in the deployment.}
        \label{subfig:testbed-graph}
    \end{subfigure}\quad
    \begin{subfigure}[h]{0.3\linewidth}
        \includegraphics[width=\linewidth]{figs/loss-rates/loss_rate_plot.png}
        \caption{Distribution of mean loss rates among directional links.}
        \label{subfig:testbed-lossrates-cumulative}
    \end{subfigure}\quad
    \begin{subfigure}[h]{0.3\linewidth}
    \includegraphics[width=\linewidth]{figs/loss-rates/custom_loss_probability_plot-no-annotations.png}
    \caption{Loss rates between nodes. Bars show the directional loss rates in terms of the mean and standard deviation over averaged 10 minute intervals.}
    \label{subfig:testbed-lossrates-links}
    \end{subfigure}\vspace{-0.1in}
    \caption{Packet loss rate measurements from the inter-building test bed deployment.}
    \label{4}
\end{figure*}



% Figure starts
\if 0
\begin{figure*}[t]
\raggedleft
\begin{minipage}{0.50\textwidth}
    \raggedleft
\begin{subfigure}{0.49\textwidth}
    \raggedleft
\includegraphics[width=\textwidth]{figures/1.pdf}
\caption{Something}
\label{fig:1}
\end{subfigure}
\begin{subfigure}{0.49\textwidth}
    \raggedleft
\includegraphics[width=\textwidth]{figures/2.png}
% \vspace{-0.1in}
\caption{Something.}
\label{fig:2}
\end{subfigure}
\caption{Some}\vspace{-0.1in}
\label{fig:simResults}
\end{minipage}\hfill
\begin{minipage}{0.25\textwidth}
\includegraphics[width=\textwidth]{figures/3.png}
\vspace{-0.28in}
\caption{Something.}
\label{fig:3}
\vspace{-0.1in}
\label{fig:simResults2}
\end{minipage}\hfill    
\begin{minipage}{0.25\textwidth}
    \raggedright
\includegraphics[width=\textwidth]{figures/4.png}
\vspace{-0.28in}
\caption{Something. }
\vspace{-0.1in}
\label{fig:4}
\end{minipage}
\end{figure*}
\fi
% Figure end



% figure Ends
%\subsection{Small-Scale Evaluation}\label{subsec-evaluation-1}

%\subsubsection{Packet loss rate measurements}
To validate both our algorithm implementation and underlying assumptions about Wi-Fi connectivity, we built a hardware testbed using Hak5 WiFi Pineapple Mark VII devices~\cite{hak5}. The Pineapple has three 2.4~GHz Wi-Fi radios and a single-core MIPS processor. Being based based on commodity hardware, similar to that which one would find in any consumer home Wi-Fi/router, it is a suitable choice for building out a testbed for \name.
Further, as the Pineapple runs modified OpenWRT~\cite{openwrt}, it is flexible and compatible with upstream OpenWRT.

To estimate packet loss rates between buildings, we deployed eight Pineapples devices across 3 buildings on a university campus.
We placed the devices across different floors in nearby buildings and configured one of their wireless network interfaces as a meshpoint.
Each device broadcasted a single UDP packet with a unique identifier over a dedicated 802.11 meshpoint interface every 5 seconds and logged these transmissions.
Simultaneously, all Pineapples listened on the same interface for broadcasted packets, and logged the unique values and timestamps of received packets.
%Received and sent packet identifiers were compared between all potential directional links.

After taking measurements over the course of two days, we evaluated the directional links between each device.
Figure~\ref{subfig:testbed-graph} shows each device has partial visibility of the mesh where at least one in 100 packets are received.
Figures~\ref{subfig:testbed-lossrates-cumulative} and \ref{subfig:testbed-lossrates-links} show loss rates measured across the mesh.
Taking 10-minute averages of loss rates over the two day of observations, we find the median loss rate to be approximately 20\%.








==> sections/hardware-eval.tex <==
\section{Hardware Evaluation}
\label{sec:hardware-eval}
To validate both our algorithm implementation and underlying assumptions about access point connectivity, we built a hardware test bed of 100 Wi-Fi nodes.
We opted for the Hak5 WiFi Pineapple Mark VII \cite{hak5} as the choice of hardware.
The Pineapple has three, 2.4~GHz Wi-Fi radios and a single core MIPS processor.
We were motivated to select this device as the device choice for our test bed as it is based on commodity hardware, similar to that which one would find in any consumer home Wi-Fi access point or Wi-Fi enabled router.
Further, as Hak5 developed the Pineapple as a penetration testing tool with an operation system based on OpenWRT~\cite{openwrt}, it is highly flexible and is compatible with upstream OpenWRT.

With this test bed we wanted to answer the following questions:
\begin{itemize}
    \item \textbf{Large scale emulation}: How does the simulated performance of our algorithm change when using real packet transmissions and receptions, versus using an RF model?
    \item \jl{Should we report packet loss rates measured by the testbed?}
    \item \textbf{Packet loss rate}: What is the approximate packet loss rate that occurs between access points in the same building and access points in different buildings?
    %\item \textbf{Performance}: What are the performance demands of our algorithm? Will our algorithm perform well on commodity hardware?
    \item \textbf{Large scale emulation}: How does the simulated performance of our algorithm change when using real packet transmissions and receptions, versus using an RF model?
\end{itemize}

To answer these questions, we deployed the Wi-Fi Pineapples in different locations and configurations.

\\
\noindent
\textbf{Test Bed Mesh Emulation}:

==> sections/micro.tex <==
\section{Micro-Benchmarks}


==> sections/routing.tex <==
\section{Building Routing}
\label{sec:routing}

%\oc{@Hari, how do you want to talk about packet headers? We currently have 21 bytes: (4 bytes for each block id - destination, sender, next waypoint, last waypoint + 4 bytes for in-building rank + 1 byte for edit count}
%\cl{Should we add a section 4.6 - Packet Header Design?}
%\hb{We are presenting this as "we want to use a map", but that is not the goal. The goal is a scalable routing protocol for static and mobile Wi-Fi devices. I suggest presenting the solution more logically as in "here's how using a map can help with scalability. Do not assume that the reader has bought into the idea of a map. Also, need to clearly explain why the solution scales.}

%As we start to utilize a map, a natural question emerges, can a packet be routed the same way that humans use a map to find a path to a given destination? Our system builds off of this idea and considers that when a human drives through a city, they go intersection by intersection, deciding which next intersection to head towards. In the same way, \name\ goes through each intermediate building, going hop to hop, deciding the next building it should go through. 

Routing is a traditionally well-studied problem with rich literature \cite{XXX}. However, previous work largely considers dealing with routing between each individual node. These protocols often require some out-of-band information (i.e. GPS) for each individual node or transmit control messaging information between each node. To keep routing information updated, these protocols largely require some form of updating or continual messaging as mobile devices continue to move throughout the network. As the number of devices in a network scale, collecting this information, maintaining this information, and relaying this information between nodes becomes extremely challenging. All together, when millions of devices are present in a network, handling any information for each separate node becomes extremely cumbersome and will not scale to practical, realistic deployments. 

Additionally, mobile nodes and Wi-Fi access points are highly constrained. Many of these devices have high loss rates with neighboring links. This is worsened by the fact that wireless spectrum is limited, leading to retransmissions of packets wasting crucial limited bandwidth. What's worse, if a packets fails to deliver, many higher-layer networking protocols will often retransmit failed packets, causing a dropped packet to re-traverse the network and create more congestion. 

Hence, \name\ should design a new routing scheme which:

\begin{enumerate}
    \item \textit{Requires a constant amount of information to be maintained by each device. In particular, the content a device stores should scale well with respect to the number of devices in the network.}
    \item \textit{Minimizes the number of retransmissions by picking a route which prioritizes the likelihood of a packet being received even if the selected route potentially requires more transmissions}
    \item \textit{Is resilient to device failures if a certain group of devices are incapable of participating in the network}
\end{enumerate}

\subsection{Observations and Design Choices}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\linewidth]{example-image-duck}
    \caption{Graph of a Building Map}
    \label{fig:buildingMapGraph}
\end{figure}

In contrast to previous work, we take a new approach which gathers information about a group of nodes at once, finding out information about buildings. This gives us two key advantages: (1) buildings are likely to have dense deployments of both Wi-Fi access points and users with mobile devices and (2) we can use building placement data to gather information about neighboring buildings. By using city maps with detailed building information, the precise geographic footprint and area of a building and the number of floors and their heights can be obtained before any network usage. Accurate maps are often collected and maintained by organizations and municipalities using satellites and drones to collect accurate map data up to an accuracy of XXX \cite{XXX}. Another unique advantage of building information is that buildings rarely change on the time span of a network being operational. This is in contrast to node-level information that changes often and is subject to numerous external environmental factors.

We formulate this routing problem as a centralized graph problem. In our proposal, a centralized server will first create a series of per-device routing tables that will be distributed to each device. In our formulation, we consider the geography of a building and the distance to neighboring buildings. This problem must be solved before the deployment of the network and can only consider information represented in the original building map.   

%Our graph problem can additionally be naturally extended to support more information about the link quality between different buildings and other external information.   

\subsection{Graph Formulation} 
We begin by describing the construction of the graph $G(V, E)$ that captures information about each building in the network, and the ability to connect between buildings. Suppose we have $N$ buildings represented by $B=\{b_1, b_2,...,b_N\}$. In Figure (\ref{fig:buildingMapGraph}), each element of the set $B$ will become a unique vertex represented by each building's unique building ID.

Given the graph with vertices $V$, an edge is equivalent to the expected connection between one building to another. However, we must account for the cost associated with selecting a hop from one building to the next. To emphasize minimizing risk in the network, we select each edge weight, $w(e)$ as the closest distance between two buildings $(b_1, b_2)$. We then prune edges $E$ that are greater than greater than the largest transmit distance of the network. We select distance as the edge weights in the graph because this information can be easily calculated between all neighboring buildings and is easily able to represent the connectivity of two arbitrary buildings. \oc{Should we mention the cost of doing this? It's very cheap tbh. takes like under a minute on a city as dense and big as Tokyo}




%maps give us 1. dense deployments of acess point, neighboring buildings, accurate routing tables

%We can exploit this to construct a routing map because we can construct information because buildings r dense and neighboringing 

%Many maps contain external information which can be extremely useful during disaster scenarios with some maps containing information about which buildings have installed solar panels and knowledge of which electrical companies provides power to certain buildings \cite{XXX}. 

%The unique leverage of building information is that it is coarse-grained and approximate. Often times, when setup, static nodes such as Wi-Fi access points are set up with exact information about the address where they are placed. This information can be relayed to mobile nodes trivially. Buildings tend to be very dense, often times having network connectivity throughout the whole entire building. Nodes can easily tell which Wi-Fi they are connected to and determine which building they are within, don't need a per Wi-Fi thing or anything. 

%building geography, distance between buildings, buildings have unique id, nodes know which building they are in (think having to setup nodes), location to the scale of buildings is trivial, neighboring buildings, accuracy of the building map. Companies use sophistcated devices to get well data. Through a building, you can approximate how many access points r in a building. Buildings are densely covered, often the whole building is covered. Knoweldge about the type of building (resedintial, office). Electricity, solar panels, energy supplier$

%To achieve this goal, \name\ converts an existing map, which is a series of intersections (vertices) and roads (edges), to a new building graph which contains information about potential hops a packet can take. In this building graph, each building becomes a vertex where each edge represents the ability for a transmission to occur between two buildings. In the same way where road graphs set the edge weight representing the estimated time between two intersections, our new building graph has each edge set to the distance between two buildings, representing the jump between one building to the next. 

%Each AP has access to a building graph, where buildings are represented as nodes and identified by building IDs. The edges in the building graph reflect neighboring relationships, with edge weights representing the distances between adjacent buildings. Additional attributes, such as the positions of buildings, are also available.

\subsection{Routing Algorithm}
To maximize the chance of deliverability, we design a new shortest-path algorithm, the \textbf{SafestPath}, which emphasizes minimizing the riskiness of each additional hop in the network. That is, prefer an edge with the smallest risk between a pair of buildings even if this means a path with a larger total distance. We formally define this as a shortest path in a transformed building graph, where each new edge weight $w\prime(e) = w(e)^k$, where $k$ is a hyper-parameter representing the trade-off between riskiness and load-balancing. This equation draws from the principle of limits where for large $k$, $w^k$ is greater than $\sum_{i=1}^{w-1} i^k$ because $w^k$ grows faster. The core intuition here is that when a number is exponentiated to a large $k$, the shortest path will continually select safer edges.

%In \name, we take inspiration from existing map-based routing which selects a route from a source to a destination through running a shortest path algorithm, trying to minimize the total traveled time. To do this, we propose a new shortest-path variant called the \textbf{SafestPath}, which seeks to minimize the chances a packet is lost when hopping between buildings. We define the SafestPath, as a variant of the shortest path which tries to find a route which minimizes the riskiness of each hop in the network, that is, taking the smallest distance between a pair of buildings even if this means a larger total path. Put formally, this is the shortest path where the edge weight of the building graph is transformed from $d \rightarrow d^k$ where $k$ is a hyper-parameter representing the trade-off between riskiness and load-balancing. This equation draws from the principle of limits, where for large $k$, $d^k$ is greater than $\sum_{n=1}^{d-1} n^k$ as $d^k$ grows faster.
% The core intuition here is that when exponetiated to large $k$, the exponential growth rate is becoming more sensitive to the base $d$.


When $k$ is small, the difference between edge weights becomes minimal. However, as $k$ increasingly becomes larger, the difference in edge weights becomes increasingly unbalanced as the shortest path will prefer smaller edge weights, causing densely placed buildings to receive a higher load of the network traffic, potentially creating additional congestion. In fact, as $k$ approaches infinity, all selected paths will occur on the minimum spanning tree, creating single points of failure \cite{MST}. \oc{Insert/Put in Appendix theorem proving that paths lie on the MST}

\subsection{Conduit Redundancy} \label{waypoints}
%Continuing on with the idea of routing the same way as a human drives through a city, a driver does not need to know every single intersection they pass but only the points where they need to turn. Otherwise, it would be unnecessarily tedious for the driver to remember to go straight at most intersections. For instance, imagine if someone was giving you directions and they told you every intersection keep going straight, you would be overwhelmed. Likewise, placing every single intersection into a packet requires a substantial header size. 

%Additionally, consider the following problem: imagine you are driving on a highway and the highway is unavailable between two exits, the same as if a series of buildings are down. One natural solution would be to exit the highway and take local roads, the same as a packet going slightly away from the prescribed route. Then, a driver would go back on the highway at the next entrance, continuing on the route, the same as a packet arriving at a certain set point and then resuming this prescribed path. Part of \name\'s design is to opportunistically achieve this same functionality. 

%first decide what pacths to pick, the natural thing to pick is distance between buildings
% imagine some transmit range, can imagine some things are connected, can be additive, cite roofnet, that just using distance means that you may pick packet loss rates
%roofnet considers all lins to get link metrics, but periodic
%looking for alternative approach is to bias the paths we select to have shorter range, rather than simply the distance but using a function of the distance. A function we can use is d^k where k is a hyper parameter, we observe that when the big links. We've experiment, we'll get k=10 works well. define it this way. 
%if we built this path, we don't know where devices are. Instead of constructing unicast packets, we want to broadcast (with suppression with later) so that if they're around builds they rebroadcast, if not they don't
%not computing paths amongst devices. contrast to, what we get is scalable routing. don't know where the devices r, a path becomes a series of condiots
One of the key goals of the design of \name\ is to design a system that is resilient to failures and imprecise information. While SafestPath minimizes the risk of a packets' ability to hop between buildings, the devices within two neighboring buildings might not be connected or even some devices within a building might not be operating. Hence, we present a \textbf{Conduit}, which is an approximation of the original SafestPath with an added degree of resiliency which allows for a deviation of the original route given the realization of a calculated path when a packet attempts to traverse the pre-planned route. Formally, a conduit is defined as a rectangle with width $w$ between the centroid of two buildings, $b_1$ and $b_2$. We define these buildings as \textbf{Waypoint Buildings}. A conduit ensures that all buildings in the original calculated SafestPath will be contained. 

To calculate the start and end waypoints of a conduit, we start at a source node $S$ in building graph $G$, and progressively test if for each element in the route, $k$, if all nodes in the route are within a rectangle from $S$ to $k$. If not all elements in the route can be fit within the rectangle, a waypoint is drawn at this turning point and this process is repeated starting at this new point. This process ensures that all buildings in the original route are within the conduit defined by the new waypoint route. 

%To create a conduit, we consider two buildings, one previous, $B_p$, and  $B_c$ (for prev and current), we draw a rectangle of width W with the centroids (or centers) of these two buildings (projected on to the road plane)  at the midpoints of the rectangle's width, with the rectangle's length equal to the distance between the two buildings, and all buildings within this rectangle are in the conduit defined by these two waypoints? Assuming what I said is correct, I don't see how Eq(1) is saying the same thing?

%To achieve this, \name\ finds essential points in a given route, called \textbf{Waypoint Buildings}, these are buildings that represent an essential or turning point in a route. These are different for each given source, destination pair

%through due to lack of knowledge for availability of wireless devices inside the building. In fact, under some circumstances, the entire building may fail to participate in the network. This will eventually break the path we computed, causing a single point of failure at the building level. However, other neighboring buildings around the point of failure can still be available. Therefore, one natural solution to this problem is to "detour" the packet in the nearby region, and come back to the safest path after surpassing the failed building.


\oc{If we have time, I have an idea to handle a broken waypoint...}

\subsection{Routing Table Distribution}
Given the global building graph $G$, the centralized server must create a minimum set of knowledge for each building of the graph. Once at the waypoint, the devices in the building need to know the next waypoint to forward to so that the packet travels along the planned SafestPath to the destination. However, it is infeasible to store every single possible destination information as an entry in each device's routing table due to memory constrain.

\subsubsection{Routing Address Assignment}
To mitigate the memory problem, we observe that destination buildings that are geographically close to one another are likely to share the same next waypoint along the path. This allows us to reduce the table size by grouping entries using a hierarchical spatial clustering algorithm. Our solution mimics the properties of both real-world addressing and IP-subnet addressing. Addresses are assigned by recursively dividing the map in half along both the x and y axes, repeatedly creating four grids a necessary desired level of granularity is achieved. The BLOCID of a building is then constructed as a chain of prefixes representing the finest grid in which the building is located, followed by a suffix that uniquely identifies each building within that grid. This approach mimics the properties of IP subnet masks by aggregating entries that share the same initial prefixes, effectively reducing the table size through using existing IP-based routing table compression techniques~\cite{gabor_ip_forwarding_compress, elliot_compression, yang_compression, richard_compression}. 

%This approach assigns a set of building location IDs (BLOCIDs) to buildings and organizes the routing table into compact clusters. Although various hierarchical spatial clustering algorithms~\cite{Malzer_2020, carvalho2009spatial, murtagh2012algorithms, assuncao_skater, chavent2018clustgeo} are available, we opt for the simplest approach: the 4-grid clustering method that is similar to the approach used by GLS~\cite{gls}.

%The problem with the current approach is that it requires knowledge of the whole entire route ahead of time, the same as having to remember a series of directions throughout your whole journey. This becomes harder as the city scales. Imagine having to remember each turn through a large city, the same as having to put all of the information about numerous waypoints into a packet header. Instead, \name\ desires a system which tells you at each turn, what the next turn will be. This is our vision with the creation of routing tables. Instead of prescribing the route ahead of time, each waypoint looks at their own routing table and gives only information about the next place to turn at, just like driving on a road with a sign at an intersection saying which way to turn to get to a destination. 

\subsubsection{Global Algorithm}
To calculate these routing tables, \name\ uses a centralized server to compute each node's routing tables and then distributes them out to each building:

\begin{enumerate}
    \item Calculate the SafestPath from each source to each destination
    \item Find the first waypoint in each calculated source, destination route
    \item Set the first waypoint as the next hop for the destination in the source's routing table
    \item Compress similar destinations to minimize the routing table size (see below) 
\end{enumerate}



\begin{figure}[t]
    \centering
    \includegraphics[width=0.3\textwidth]{figs/BLOCID.png}
    \caption{\small Illustration of 4-Grid Clustering and BLOCID Assignment}
    \label{fig:blocid}
\end{figure}


%In Table~\ref{tab:routing_table_compression}, we present an example of compressing a routing table using BLOCIDs. The first four entries share the same next waypoint, identified by the BLOCID $1101001101$, while the destination grids are specified as $001100/6$, $001101/6$, $001110/6$, and $001111/6$. This demonstrates that to route toward the coarser grid $0011/4$, it is sufficient to use the same next waypoint $1101001101$. As a result, we can combine these four entries into a single entry: $(1101001101, 0011/4)$.

\iffalse
\begin{table}[ht]
    \centering
    \begin{subtable}[t]{0.45\textwidth}
        \centering
        \caption{Uncompressed Routing Table}
        \begin{tabular}{|c|c|}
            \hline
            Next Waypoint & Dest. BLOCID Prefix \\
            \hline
            1101001101           & 001100/6 \\
            1101001101           & 001101/6 \\
            1101001101           & 001110/6 \\
            1101001101           & 001111/6 \\
            1101011000           & 10110100/8 \\
            \hline
        \end{tabular}
    \end{subtable}
    \hspace{0.05\textwidth}
    \begin{subtable}[t]{0.45\textwidth}
        \centering
        \caption{Compressed Routing Table}
        \begin{tabular}{|c|c|}
            \hline
            Next Waypoint & Dest. BLOCID Prefix \\
            \hline
            1101001101           & 0011/4 \\
            1101011000           & 10110100/8 \\
            X                    & X \\
            X                    & X \\
            X                    & X \\
            \hline
        \end{tabular}
    \end{subtable}
    \caption{Compression of Routing Table with BLOCIDs}
    \label{tab:routing_table_compression}
\end{table}
\fi
% Given a building route \(R = (b_1, b_2, \ldots, b_n)\) and the conduit width $W$, the compressed building route $R^*$ is:
% \begin{equation}
% %\small
% R^*(R, W) = \left\{ b_i \in R \mid \texttt{Relay}(b_i, b^*_{prev}, W) \right\}
% \end{equation}
% where $\texttt{Relay}(b_i, b^*_{prev}, W)$ is a predicate that is true when a building $b_i \in \mathcal{R}$ is the last one that forms a conduit with the previous waypoint building $b^*_{prev}$, covering all buildings between them in $R$.

\iffalse
\begin{algorithm}[!t]
\DontPrintSemicolon
    \KwInput{A building route ${B}$, where $B = [b_1,b_2,...,b_{n-1},b_n]$}
    \KwOutput{A list of waypoints ${W}$, where $W = [w_1,w_2,...,w_{k-1},w_k]$}


    \nonl\textcolor{cyan}{ \(\triangleright\) \textit{Initialize the waypoint list}}\\
    ${W}$ = empty list\\
    
    \nonl\textcolor{cyan}{ \(\triangleright\) \textit{Append source building ID as first waypoint}}\\
    ${b_{source}}$ = $self$.building\_id\\

    ${W}$.push\_back(${b_{source}}$)\\
    \nonl\textcolor{cyan}{ \(\triangleright\) \textit{If we make two back-to-back buildings as waypoints, it is always valid and no need to test, so we start from the second building}}\\
    \Loop ($b_i\in{B}, i\geq2$:)
    {
    \nonl\textcolor{cyan}{ \(\triangleright\) \textit{Check the feasibility of waypoint placement at the current building given the last valid waypoint}}\\
    ${w_{start}}$ = ${W}$.tail()\\
    ${w_{test}}$ = ${b_i}$\\
    ${W_{test}}$ = make\_list($[w_{start}, w_{test}]$)\\
    
    \nonl\textcolor{cyan}{ \(\triangleright\) \textit{All buildings starting from the last waypoint building to the current building are tested}}\\
    \Loop ($b_m\in{B[w_{start} : w_{test}]}$:)
    {    
        \If ({$b_m$.should\_broadcast(${W_{test}}$) is $false$:})
        {
        \nonl\textcolor{cyan}{ \(\triangleright\) \textit{The waypoint placement at current building fails, we place the waypoint at the last successfully tested building}}\\
        ${W}$.append($b_{i-1}$)\\
        break
        }
    }
    }
    \nonl\textcolor{cyan}{ \(\triangleright\) \textit{Add destination as the final waypoint if it has not yet been added}}\\
     \If ({$B$.tail() not in $W$:})
     {
        ${W}$.append($B$.tail())
     }
    
    return ${W}$
\caption{${compress(B)}$}
\label{alg:header_compression}
\end{algorithm}
\fi
%Continuing on with the idea of routing the same way as a map does, a person driving a car does not need to know the location of every single intersection along a path, they only need to know when to turn. In the same way, a packet should only contain information about when to change paths and should 



\iffalse
In traditional map routing, a source calculates a path to the destination using some variant of a shortest path graph algorithm over the expected arrival time. However, when applied to packets, which travels by a series of broadcast, minimizing the distance traveled will lead to a few challenges:

\begin{enumerate}
    \item The shortest path is not necessarily the most reliable path. This means that a source must calculate ahead of time, a path which must work for the whole entire route 
\end{enumerate}

1. 

2. Packet Header Encoding As the network expands and the distance between source and destination buildings increases, the number of building hops grows. This leads to a larger number of building IDs stored in the packet header, causing the header overhead to become excessively large and inefficient.

3. Source Computation Expense APs typically have limited computational capabilities. Calculating the shortest path incurs a complexity of $O(V+E\cdot logV)$, which can place a significant burden on the source node in large networks.
\endif



%\cl{Update the transition after the system design section is complete.} With the postbox design, the routing problem becomes how to deliver the packet from the source AP to the destination AP, where in the common case the two APs are in two different buildings. However, this problem is far from trivial given that we are not allow to flood any control packet or rely on any per-node geographical information. For the network to scale well, we should also consider reducing, as much as possible, the metadata sharing and the amount of states maintained by each node.

% \subsection{Source Routing - Shortest Path}
% Explain a naive source routing solution here, and list the problems to be solved by our final routing solution.
%In our design, the same building graph of a city is distributed to each AP. In the building graph, the nodes contain unique building IDs for different buildings, and edges weights are distances between buildings. \cl{remember to report the building graph memory size somewhere}
%As a simple solution, a source AP can perform source routing and construct the building route by a set of building IDs. 
%The source can obtain this building route by running a Dijkstra shortest path algorithm over the building graph. 
%Every intermediate AP can match their own building ID with the building route in the packet header. 
%Then, the intermediate AP will broadcast the packet if it is inside the building specified by the source AP. 
%As a result, the packet will hop between buildings and finally reaches the destination building/postbox. 
%This naive approach may achieve end-to-end delivery, but leads to the following problems.

\begin{enumerate}
    \item \textbf{Route Prediction.} The shortest path is not always the safest path. \hb{Have we defined "safest" earlier? What does it mean?} Moreover, no recovery is available since we remove flooding of the control packet and reduce metadata sharing. This means if the packet is unable to hop from a building to the next building, we lose the packet permanently midway through the route.
    \item \textbf{Packet Overhead.} As the network size expands and buildings are spatially more separated, the number of building hops will increase. This results in more buildings IDs being stored in the packet header, and makes the overhead in the packet header unreasonably large. 
    \item \textbf{Building Participation.} The naive approach assumes every building on the building route will participate. In the case where some buildings are unable or unwilling to participate, the route will break and the packet will be lost.
    \item \textbf{Transmission Overhead.} Although network-wide flooding is prevented, the packet is still flooding within each building. This causes a lot of unnecessary transmission within a building. For large buildings, not all of the APs need to broadcast the packet to pass the packet from one side of the building to the other side.
    \item \textbf{Computation Expense.} APs usually have very limited computational power. Computing the shortest path has a cost of $O(V+E\cdot logV)$. For large network, this can put a lot of burden on the source node.
\end{enumerate}

To solve the problems above, we will present in the following sections our full routing solution: \circled{1} Safest Path Source Routing \circled{2} Waypoints and Conduit \circled{3} Suppression \circled{4} Map Pre-processing and Routing Table

\subsection{Source Routing - Safest Path} \label{safest_path}
The safest path source routing targets to address the \textbf{route prediction} problem. The shortest path computed over the edge weight as building distance is not necessarily the safest path. For example, suppose the transmission range of an AP is about 60 meters, consider the following example with two paths from source building to destination building:
\begin{enumerate}
    \item \textbf{Path 1}: Eight 20-meter edges
    \item \textbf{Path 2}: Two 59-meter edges
\end{enumerate}
Shortest path algorithm will choose the second path because of its lower total distance. However, the second path is at the limit of the AP's transmission range. Unless both APs are placed by the windows of their buildings, the packet is at extreme risk to be lost in this transmission. Given that the exact AP location inside a building is unknown and the packet loss rate will ramp up very rapidly towards the limits of the transmission range \cite{Yan's model and other error model}, the source routing algorithm needs to pick a path with minimal number of outstanding risky edges in the building graph (i.e., minimizing per-hop distance). Intuitively, this path can be found by raising the all the edge weights to the power of $n,n>1$ to amplify the difference of distances between buildings and then run the shortest path over the building graph. As the power $n$ becomes large enough, the resulting path will stay away from the transmission range limit as possible. Formally speaking, among all possible paths, we need to find the path that minimizes the maximal edge (riskiest edge) on the path. This is also referred as the minimax path~\cite{minimax graph problem}. 
% On top of it, if the maximal edges of two path are equal, the next maximal edge will be used for tie-breaking iteratively.
On top of it, we also require this minimax property to be satisfied for any subset of this path.
We define the path found above as the safest path \cl{Add a footnote saying that the safest path may not be the probabilistically safest, the link weight used here is only the building distance, there can be different heuristic for link weight that better approximate the probability of transmission including building area of adapting a better wireless model}. The formal algorithm to find the safest path will be a modified Prim's algorithm~\cite{prims}, which is originally invented for computing the minimum spanning tree. In Section \ref{routing_table}, we will further prove that, given all edge weights are distinct, the safest path from any source to any destination is always on the minimum spanning tree of the graph.


\cl{Move this algorithm to appendix if needed}
\begin{algorithm}
Graph $G = (V, E)$ with weights $w(e)$\;
Source $S$\;
Destination $D$\;
PriorityQueue $PQ$\;
Set $Visited$\;
Set $SafeEdges$

\ForEach {edge $e = (S, v)$ in $E$}{
    $PQ$.add($w(e)$, $S$, $v$)
}

\While {$PQ$ not empty} {
    $w(e)$, $u$, $v$ = $PQ$.extractMin\;

    \If {$v$ not in $Visited$} {
        $SafeEdges$.add($u$, $v$)\;
        $Visited$.add($v$)\;

        \If {$v$ == $D$} {
            $G' = (V, SafeEdges)$
            return $Path(G', S, D)$
        }
        
        \ForEach {edge $e = (v, q)$ in $E$}{
            \If {$v$ not in $Visited$} {
                $PQ$.add($w(e)$, $v$, $w$)
            }
        }
        
    }
}

return \textit{no path exist}\;

\caption{Safest Path}
\end{algorithm}

\subsection{Waypoints and Conduit} \label{waypoints}
The waypoints generation and the idea of conduit help address the \textbf{packet overhead} and \textbf{building participation} problem. By storing all building IDs in the packet header and then asking every building in the header to participate in forwarding is problematic. It results in excessive packet header size and packet loss if any building on the route does not participate. Since the building route will generally move in one direction towards the destination building or towards a region where the packet can route through a void in the map, we choose a subset of buildings in the building route as waypoints (WPs), and define a conduit based on the WPs selected. Effectively, a conduit is a rectangular region that begins and ends on a \emph{waypoint building}. It has a length $L$ and width $W$, where the length is a user defined constant and width is the distance between waypoint building centroids. Now instead of only buildings on the building route transmitting, all buildings within the conduit should all participate in forwarding the packet. In most cases, as long as a subset of buildings in the conduit forwards the packet to the next waypoint, the packet can get through. As a result, this largely mitigate the building participation problem. Moreover, encoding the routes as waypoints also serves as a compression of the original building route, which reduces the packet header size massively. In our simulation over large cities, the waypoint encoding compresses the original route by XX\% to YY\%. To achieve loss-less compression, where all the original buildings are retained within the conduit, we propose our waypoint selection algorithm as follows. 

Given a building route \(R = (b_1, b_2, \ldots, b_n)\) and the conduit width $W$, the compressed building route $R^*$ is:
\begin{equation}
%\small
R^*(R, W) = \left\{ b_i \in R \mid \texttt{Relay}(b_i, b^*_{prev}, W) \right\}
\end{equation}
where $\texttt{Relay}(b_i, b^*_{prev}, W)$ is a predicate that is true when a building $b_i \in \mathcal{R}$ is the last one that forms a conduit with the previous waypoint building $b^*_{prev}$, covering all buildings between them in $R$.

We acknowledge that, in exchange of smaller packet header and more robust end-to-end delivery, flooding all buildings in the conduit will lead to more excessive transmissions, and hence, a suppression scheme will be introduced in Section \ref{suppression}.

\subsection{Suppression} \label{suppression}
The suppression helps address the \textbf{flooding} problem. Currently, we have two types of flooding problem: \circled{1} In-conduit Flooding due to waypoint scheme introduced in section \ref{waypoints} \circled{2} In-building flooding where all nodes in the building need to broadcast. In fact, flooding is inevitable without metadata sharing due to the lack of control packets to suppress transmission. Here we will present two delay-based suppression schemes that exploits the commonly owned building map knowledge, which contains the metadata sharing to only one hop, and minimizes the amount of metadata to be shared. The proposed suppression scheme will work for solving both flooding problems by changing the heuristic function for computing the delay.

\subsubsection{Inter-building Suppression}
We firstly notice that only a subset of buildings needs to involve in the transmission to achieve end-to-end packet delivery. Therefore, some buildings in the conduit can completely suppress their transmission to save power and bandwidth. Here we leverage the fact that all the APs have the common view of the building map for a city to minimize the amount of metadata shared. From there, the broadcasting APs can encode their building ID in the packet header, and the receiving APs in other buildings can independently compute the same set of all neighbor buildings from the sender buildings using the map. Then every receiving node will rank all neighbor buildings based on the distance to the next waypoint, drop buildings that drive the packet further away from the next waypoint, and computes a delay based on its own buildings rankings. To maximize per-hop distance, if a node's building is closer to the next waypoint, its timer should be shorter. After a time out on the delay and no other buildings have broadcast the packet, the receiving node should turn into a broadcasting node because it shows no other neighbor buildings closer to the next waypoint is participating. Otherwise, if the receiving node hears the packet, this shows there is a participating building in the transmission range that is closer to the next waypoint. In this case, the receiving node should turn into a suppressed node, and not re-broadcast the packet that has already gone further towards the next waypoint. 

Notice that for this suppression scheme, only the sender building ID is shared as metadata, so it is smaller enough to be encoded as a field inside the data packet header instead of sharing it through a control packet. Also, due to lack of metadata sharing beyond one hop, we will experience hidden terminal problem, however, the propagation of the hidden terminal problem will be contained by the conduit, and have multiple paths that are spaced out in the conduit also increase the redundancy while adding a small number of extra transmission overhead.

\begin{figure}
    \centering
    \includegraphics[width=0.3\textwidth]{figs/Inter-Building_Suppression.png}
    \caption{\small An illustration of the inter-building suppression protocol. Building $\alpha$ and $\beta$ drop the packet since they are further away from the next waypoint as compared to the sender building. Building $\gamma$, $\eta$, $\varepsilon$, $\theta$ use the building graph to independently compute their own rank among all neighbor buildings.}
    \label{fig:suppression-inter-rank}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.3\textwidth]{figs/Inter-Building_Suppression_Multipath.png}
    \caption{\small Based on the ranks, building $\theta$ will first times out on its delay, and broadcast the packet. Building $\eta$ and $\varepsilon$ receive the broadcast, and suppress their pending transmission. Building $\gamma$ is a hidden terminal to building $\theta$, and also broadcasts the packet after its delay times out.}
    \label{fig:suppression-inter-multipath}
\end{figure}

\subsubsection{Intra-building Suppression}
The intra-building suppression will apply the same delay-suppress scheme. Unlike the inter-building scenario, where the node's building can be precisely located on the map, the nodes are unable to acquire precise location information inside a building to distinguish themselves from each other. As a result, we estimate the intra-building positions based on the node's proximity to other buildings. In warm-up time, every node will simply flood within the building. As the network runs, some nodes may hear the other buildings' data packets. These nodes will record these building IDs and compute a proximity score based on the number of building recorded and the closeness of these buildings to the next waypoints. Finally, the nodes in the same building will generate the delay based on this proximity score along with a random jitter to distinguish nearby nodes. From here, the same delay-suppress scheme from inter-building suppression will apply.

\begin{figure}
    \centering
    \includegraphics[width=0.3\textwidth]{figs/Intra-Building_Suppression.png}
    \caption{\small To be Added.}
    \label{fig:suppression-intra-rank}
\end{figure}

The delay-based suppression scheme is shared across inter-building and intra-building scenario. The only difference is the variable used to compute the rank and delay. The inter-building suppression uses the precise building location and the intra-building suppression uses the proximity score.

\cl{it will be great if we can share a sequence of packet propagation plot showing the effect of each technique above}

\subsection{Map Pre-processing and Routing Table} \label{routing_table}
Map pre-processing and routing table helps further resolve the \textbf{packet overhead} problem and reduce \textbf{computation expense} for the source node and the intermediate nodes. Although source routing is possible via the routing design in section \ref{safest_path}, \ref{waypoints} and \ref{suppression}. It still has a packet header that scales with the size of the map. For larger cities, this can again be problematic. Additionally, the computation expense for the source node to generate the safest path is high. This can slow down the packet generation at the source. Again, we leverage the knowledge of the building map, and propose a routing table design that pre-processes the map which results in a constant-size packet header and faster source packet generation. 

We first make an observation that for all the buildings on the safest path $P$ from source $S$ to destination $D$, if any of them computes a intermediate safest path $P'$ to the destination $D$, this intermediate safest path $P'$ will be on the original source-originated safest path $P$. This can be shown by all safest path are on the minimum spanning tree (MST) of the graph, so all intermediate buildings will share exactly one route on the MST to the destination building.  
% \subsubsection{}
% A brute force solution will be, in map pre-processing phase when centralized computation is available, generating all routes from any source building to any destination building, and ask each source node to cache the routes from its source building to all destination buildings. Although the heavy computation cost can be compensated by the high performance data center, this approach will be costly in memory

% Theorem 1: $Safest\_Path(S,D) = Path(MST, S, D)$
% \cl{remember to mention the uniqueness of the mst given our floating point values}

% Proof: The proof is essentially a proof by contradiction. Assume there exist a safest path P' that is not on the MST. Then we find the maximal edge on Path(MST, S, D), disconnect this edge, and reconnect this component to the graph using the edge on P', which is smaller than the removed maximal edge (Need to elaborate why this connection exists). This results in a spanning tree with smaller total weight, which shows that the original MST is not a MST. Contradiction.

\begin{theorem}
Given edge weights are all distinct, any safest path defined in Section \ref{safest_path} is the on the minimum spanning tree (MST) of the graph. 
\end{theorem}

\begin{proof}
Proof by contradiction. Since all edge weights are distinct, the MST is unique. Assume, from source $S$ to destination $D$, there exists a safest path $P'$ that is not on the MST. Firstly, we find the path $P$ from $S$ to $D$ on the MST. Then we locate the maximal edge $e_{max}$ on $P$, and remove this edge from the MST. This will partition the MST into two MSTs, $MST_1$ that contains node $S$ and $MST_2$ that contains node $D$. Since safest path $P'$ from $S{\in}MST_1$ to $D{\in}MST_2$ exists, it must travel through an edge $e_{p'}$ that connects $MST_1$ and $MST_2$. As $P'$ is the safest path, $e_{p'}{\leq}e_{max}$. Now we create a new spanning tree $MST_p$ by connecting $MST_1$ and $MST_2$ with $e_{p'}$. Since all other edges are the same, and $e_{p'}{\leq}e_{max}$, the new spanning tree $MST_p$ have with either smaller or equal total weight, \hb{didn't understand the last clause -- ``have with either smaller or equal total weight'' -- what does this mean?} which shows that the original MST is not a MST or not unique, and hence, leads to a contradiction.
\end{proof}

In our building graph, all building edge weights are floating point numbers, so there is nearly zero probability for two edges having the same weights. Therefore, all of our intermediate safest path will be on the source generated safest path. From this, we can generate routing tables that only store the next waypoint to the destination because all subsequent waypoints will generate their next waypoint in the same sequence as the source routing waypoint route. Before the deployment of the system, we can utilize centralized compute power to generate the MST of the building graph, and compute the next waypoint needed for each source to reach each destintaion. Eventually each source will have a routing table of (next waypoint, destination) pairs. \cl{add an example routing table here}.

Simply adding one entry for each destination can lead to an over-sized routing table. However, since most destination buildings that are spatially close to each other will likely share the same first waypoint from the source, we can use a hierarchal spatial clustering algorithm to assign a set of building location IDs to the buildings, and group entries in the routing table to compact its size. While other hierarchal spatial clustering algorithms exist ~\cite{may be cite some clustering algorithm}, we will use the simplest GLS~\cite{gls} grid clustering to show the ... \cl{needs result on how compact the routing table can be} 

\cl{also talk about the MST congestion problem}

==> sections/system-design.tex <==
\section{\name\ Overview and Goals}
\label{sec:system-design}

\hb{City. We don't have results elsewhere.}

\hb{Can we show some feasibility results for different Wi-Fi ranges in a few diff cities? The goal is to show the size of connected islands assuming buildings have Wi-Fi in them for different Wi-Fi ranges and different degrees of penetration of participating Wi-Fi.}

\noindent
\subsection{Motivation}
We developed \name as a solution to realize a DFN in the context of a densely settled, metropolitan area.
A city-scale DFN supplements internet connectivity for local communications across the region when centralized internet infrastructure is disabled.

High-impact events such as natural or environmental disasters, critical misconfigurations of network assets~\cite{rogers_outage}, and cyberattacks occur with increasing frequency \cite{XXX}.
% reword with examples
In hurricanes, users may be left without internet when fiber is cut. In these circumstances, users may have power and battery powered mobile devices but be unable to communicate with the public internet.
Misconfigurations of network equipment that bring down entire ASs are relatively rare, but do occur as network complexity increases.

Deploying a DFN across a metropolitan area poses unique challenges.
In this environment, device density is high, and many clients are highly mobile.
However, the density of access point nodes \jl{check terms introduced in intro once written} in a city suggests that a large, continuous mesh of devices could be constructed without the addition of many, if any, new nodes.
Therefore, we require \name to be compatible with existing access point nodes and mobile devices so that existing wireless infrastructure in a city could be repurposed to the greatest extent possible.

% climate disasters, misconfigurations, cyberattacks

% motivate looking at wireless nodes in settled areas
% transition to the below features of a protocol that is optimized for this area
\noindent
Further, we designed \name to meet the following requirements:
\begin{itemize}
    \item \textbf{Scalability}: This protocol must be able to support an arbitrarily large number of wireless devices.  
    \item \textbf{High Deliverability:} This protocol must be able to deliver a packet from a source to a destination successfully, provided a route exists.
    \item \textbf{No Control Packet Usage:} This protocol should not use any routing messages, control packets, or probing messages so that full bandwidth may be utilized for data packet transmissions. 
    \item \textbf{Low Transmission Overhead:} Our protocol should deliver a packet with the minimum number of transmissions possible. 
    \item \textbf{No Precise Per-node Positional Information} This protocol must be tolerant of imprecise geographic positioning.
    %\item \textbf{Resiliance to Node & Building Failure}. Our system should be able to tolerate both individual nodes in the network failing and whole buildings failing
\end{itemize}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\linewidth]{example-image-duck}
    \caption{Example of Map Converted to a Building graph}
    \label{fig:map-example}
\end{figure}

\noindent

\subsection{Routing with Maps}
The goal of \name is to demonstrate a novel system design which scales to millions of nodes.
%novel protocol and routing scheme that scales to millions of nodes. 

%As described previously, geographic routing protocols for MANETs rely on local knowledge of the wireless network topology to make forwarding decisions.
Protocols for MANETs generally rely on discovery of the wireless network topology to make forwarding decisions.
Consequently, incomplete knowledge of the topology results in packets reaching voids in connectivity.
Some protocols like GPSR~\cite{GPSR} attempt to recover from dead ends by forwarding the packet around the void, but do so without knowing which direction is most optimal.
% In GPSR, once a packet has moved around the void, nodes resume forwarding the packet greedily towards the destination.
While effective at recovering from these voids, this mitigation is far from ideal as the packet may end up far from its intended destination.
We observe that if node locations throughout the network could be determined in advance of a forwarding decision, voids in connectivity could be avoided entirely while by following the most optimal, extant path.
However, in order to scale to millions of nodes such foreknowledge of node location would need to be attainable without busying the network with route discovery messages.

How does such a network make informed forwarding decisions that avoid gaps in connectivity without metadata exchange?
We find a solution in the simple realization that wireless clients and access points (together, nodes) are almost always found within or near building structures, or along roads.
Further, we note that information describing the location and geometry of buildings and roads is openly and programmatically accessible through databases like the OpenStreetMap~\cite{OpenStreetMap}.
The availability of this information allows nodes participating in a MANET to make forwarding decisions based on building placement, and by extension where nodes are most likely to be found.

\name utilizes the building and road geographical data found in digital maps to make informed forwarding decisions.
More precisely, \name works by using map navigation to avoid forwarding packets along paths where voids in connectivity are not likely to occur.
The map data does not guarantee that nodes will be present in all buildings or along all roads in a particular route, but these data help nodes avoid areas where nodes are \emph{not} likely to be present.
Using map data, packet routes plotted using building locations take advantage of stationary wireless access points~\jl{terms}, taking into account the building density or building proximity to improve route selection.
With knowledge of only their imprecise location, on the scale of a building footprint, nodes make the decision to forward/rebroadcast packets along routes that contain densely clustered buildings.
Bootstrapping knowledge of which building a node is in is possible either through explicit configuration or automatic by crowdsourcing location from nearby mobile nodes that have access to GNSS services.

In the design of \name we make the assumption that most if not all buildings contain at least a single wireless node, such as a wireless access point \jl{terms}, and larger buildings such as commercial properties and apartment buildings contain many more.
Further, we make the assumption that 2.4~GHz Wi-Fi penetrates both internal and external walls while maintaining sufficient signal strength to keep the packet error rate low \jl{testbed results are good to reference here}.

% To achieve these goals, \name\ relies on the core observation that most client devices and Wi-Fi access points are almost always found within buildings.

\noindent
\subsection{System Design}
\jl{move to separate section after routing or sim?} \hb{I think the use case needs to be earlier, but written succinctly -- we can cite the HotNets paper.}

\name comprises both a routing algorithm and core features that enable a class of low-throughput applications.
\name enables secure communication of small messages across metropolitan areas such as text messaging, one-to-many emergency notifications, location sharing, and offline commerce even when the internet is not accessible.
Both mobile nodes and stationary access point nodes may participate in \name, using identical packet forwarding behavior.

\hb{Explain why we need PO boxes}
All nodes that participate in \name may serve two functions: as packet forwarding agents and application hosts.
For example, users may select stationary access point nodes to serve as destinations for their messages, like an IMAP server, so that a user's mobile device polls a device with a known location for new messages~\cite{citymesh}.
These devices serve as a user's postbox.\cite{citymesh}
We envision users exchanging public keys and postbox information out-of-band, such as over the internet before an outage, well-known hosted directory system, or in person.
A location-aware routing algorithm coupled with the ability to store and retrieve messages throughout the network serve as the primitives that enable the development of many types of applications on \name.

In terms of realizing \name on existing hardware, mobile nodes run custom applications to manage message transmission, storage, and contact book information.
These applications send and receive messages from the joined Wi-Fi mesh network to participate in \name packet forwarding.
With mobile devices it is essential that these applications carefully manage participation in the network in order to preserve battery lifetime.
Participation by these devices could be throttled in terms of packets rebroadcasted as remaining battery power falls.
Additionally, access point nodes participate in \name by running a lightweight image of OpenWRT~\cite{openwrt} that contains the necessary algorithm implementation and stored map data.
Taking advantage of OpenWRT's broad hardware support, we add new behavior to many existing access points without disabling existing functionality.
\jl{Finally, this configuration allows nodes to receive updates to the map data asynchronously as mobile nodes roam between access points.}



%makes a key observation that most devices are actually inside buildings.
% Further, we observe that detailed, up-to-date building and road positioning data are known for nearly every part of the world and are freely available~\cite{OSM}.
% This information is readily available in public map information which is continually updated while this information changes extremely sparsely. Publicly available maps typically include highly precise information about buildings and roads, including information about the polygon shape and location of buildings.

